Multimodal Knowledge Expansion

The popularity of multimodal sensors and the accessibility of the Internet have brought us a massive amount of unlabeled multimodal data. Since existing datasets and well-trained models are primarily unimodal, the modality gap between a unimodal network and unlabeled multimodal data poses an interesting problem: how to transfer a pre-trained unimodal network to perform the same task on unlabeled multimodal data? In this work, we propose multimodal knowledge expansion (MKE), a knowledge distillation-based framework to effectively utilize multimodal data without requiring labels. Opposite to traditional knowledge distillation, where the student is designed to be lightweight and inferior to the teacher, we observe that a multimodal student model consistently denoises pseudo labels and generalizes better than its teacher. Extensive experiments on four tasks and different modalities verify this finding. Furthermore, we connect the mechanism of MKE to semi-supervised learning and offer both empirical and theoretical explanations to understand the denoising capability of a multimodal student.

==> 2.related_new.tex <==
\section{Related Work}
\subsection{Semi-Supervised Learning}

\noindent\textbf{Pseudo labeling.}
Pseudo labeling, also known as self-training, first trains a teacher model with labeled data, then uses the teacher model to generate pseudo labels, and finally uses both labeled and unlabeled data to jointly train a student network \cite{lee2013pseudo,noisystudent}. Despite its simplicity, pseudo labeling methods lead to significant improvement on various tasks: image classification \cite{billion,noisystudent,metapseudolabels}, semantic segmentation \cite{zoph2020rethinking, naivestudent}, domain adaptation \cite{zou2019confidence}, etc. One important limitation of pseudo labeling is confirmation bias. Since pseudo labels are inaccurate, the student network may potentially learn these mistakes. Various methods have been proposed to alleviate this bias \cite{zou2019confidence,arazo2020pseudo,noisystudent,metapseudolabels}. However, their discussion is limited to unimodality.

\noindent\textbf{Consistency regularization.}
Consistency regularization is another important brand of SSL. Based on model smoothness assumption, consistency regularization methods constrain model predictions to be invariant to small perturbations of either inputs or model hidden states. A series of works have been proposed on producing random perturbations, such as using an exponential moving average of model parameters \cite{tarvainen2017mean}, data augmentation \cite{uda, fixmatch}, dropout \cite{bachman2014learning, noisystudent} or adversarial perturbations \cite{miyato2018virtual}. 


\noindent\textbf{Combination of various ingredients.}
To benefit from both advantages of pseudo labeling and consistency regularization, recent works \cite{Mixmatch, remixmatch, fixmatch} combine them together. In light of this, we base our learning framework on pseudo labeling and incorporate consistency regularization during training. Compared with current SSL methods, our multimodal knowledge expansion framework effectively addresses confirmation bias and provides a novel angle in dealing with this bias. 

\subsection{Knowledge Distillation}
Knowledge distillation (KD) \cite{KD,yang2019training,romero2014fitnets,tung2019similarity} is an effective technique in transferring information from one network to another. The main application of KD lies in model compression, where a lightweight student network learns from a cumbersome teacher network \cite{kdoverview}. Different from them, we expect a student model that can outperform its teacher and term this concept as knowledge expansion~\cite{noisystudent}.

Cross-modal learning is another application of KD. Cross-modal KD transfers knowledge from the teacher's modality to a student learning from another modality. A variety of methods rely on supervised learning for cross-modal transfer and thus require labeled multimodal data \cite{hoffman2016cross, nagrani2018learnable}. Another line of works develop methods in an unsupervised manner \cite{aytar2016soundnet, zhao2018through, arandjelovic2017look}. While they utilize a unimodal student from the target modality, we propose a multimodal student that better bridges the gap between source and target modalities, achieving knowledge expansion.

%A challenging scenario \HZ{our scenario?} where labels of multimodal data are not available is under exploration. To this end, a variety of methods utilize a unimodal student from the target modality in an unsupervised manner. \HZ{The last sentence is a bit weird, consider removing it.}

% In this work, propose a multimodal student that better bridges the gap between source and target modalities.

% In this work, we consider a challenging scenario where we don't have true labels for the multimodal data. To this end, a variety of methods have been developed in an unsupervised manner \cite{}. 

\subsection{Multimodal Learning} Fusing data from multiple modalities has exhibited a clear advantage over the unimodal baseline in various applications, for instance, sentiment analysis \cite{sentiment1, sentiment2}, emotion recognition \cite{emotion1, emotion2}, semantic segmentation \cite{feng2020deep,valada2019self, sagate, rgbchannel} and event classification \cite{abavisani2020multimodal}. Unlike most works that rely on labeled multimodal data, we consider a realistic yet more challenging setting: the collected multimodal data are unannotated.
% Under our proposed framework, a multimodal network trained only on unlabeled data can outperform a unimodal network trained on both labeled and unlabeled data.

==> supp1-data.tex <==
\setcounter{section}{0}
\section{Dataset and Implementation Details}
% \subsection{TwoMoon Experiment}
% We generate 500 samples making two interleaving half circles. The dataset is randomly split as 30 labeled samples, 270 unlabeled samples and 200 test data (i.e., $|D_l|=30$, $|D_u|=270$, and $|D_{test}|=200$). Note that only one feature (i.e, X coordinates) of labeled data $D_l$ is accessible, while unlabeled data $D_u$ have both X and Y coordinates as features. 

\begin{figure*}[!htp]
\centering
\centering
\subfloat[UM teacher]{
\includegraphics[width=0.3\textwidth]{fig/emo/emo-t.png}
\label{fig:emo-a}
%\caption{fig1}
}
\quad
\subfloat[NOISY student]{
\includegraphics[width=0.3\textwidth]{fig/emo/emo-um.png}
\label{fig:emo-b}
}
\quad
\subfloat[MM student]{
\includegraphics[width=0.3\textwidth]{fig/emo/emo-mm.png}
\label{fig:emo-c}
}

\caption{normalized confusion matrix test accuracy}
\label{fig:emo}
\end{figure*}

\subsection{Emotion Recognition}
The Ryerson Audio-Visual Database of Emotional Speech and Song (RAVDESS) contains videos and audios of 24 professional actors (12 female, 12 male), vocalizing two lexically-matched statements. It contains 1440 emotional utterances with 8 different emotion classes: neutral, calm, happy, sad, angry, fearful, disgust and surprise. The dataset is randomly split as 2:8 for $D_l$ and $D_u$ and 8:1:1 as train / validation / test for $D_u$. To construct the labeled uni-modal dataset $D_l$, we select images every 0.5 second of a video clip as modality $\alpha$ and train a facial emotion recognition (FER) network as the UM teacher, which classifies emotions based on images. Image-audio pairs from video clips consist of the unlabeled multimodal dataset $D_u$. We sample images as inputs from modality $\alpha$ in the same way, adopt "Kaiser best" sampling for audios and take Mel-frequency cepstral coefficients (MFCCs) as inputs from modality $\beta$. 
% Hard pseudo labels given by the UM teacher are adopted.

\subsection{Semantic Segmentation}
NYU Depth V2 contains 1449 RGB-D images with 40-class labels, where 795 RGB images are adopted for training the UM teacher and the rest 654 RGB-D images are for testing. Besides labeled data, NYU Depth V2 also provides unannotated video sequences. We randomly sample 1488 RGB-D images as $D_u$ for training the student. Soft labels of the UM teacher are adopted. 

In addition, we propose a confidence-weighted loss term in this task to further regularize the student, preventing it from overfiting to the teacher. For each sample pixel $\mathbf{x}$ and its soft pseudo label $\tilde{\mathbf{y}}$, we assign $\mathbf{x}$ with a weight $\omega(\mathbf{x})$ defined by:
\begin{equation}
    \omega(\mathbf{x}) = 1 - \frac{\sum_{k=1}^K \tilde{\mathbf{y}}_i \log \tilde{\mathbf{y}}_i}{\log K}
\end{equation}
$K$ denotes the number of classes. We then modify $\mathcal{L}_{pl}$ in Equation (4) of the main paper by applying a weight for each sample:
\begin{equation}
    \mathcal{L}_{pl} = \frac1 M \sum_{i=1}^M \omega(\mathbf{x}) \  l_{cls}(\tilde{\mathbf{y}}_i,  \mathbf{f}_s(\mathbf{x}_i^\alpha, \mathbf{x}_i^\beta;\theta_s) \label{eq:l_pl})
\end{equation}

Figure \ref{fig:conf} demonstrates one image and its confidence map (\ie, $\omega(\mathbf x)$) based on pseudo labels of the UM teacher. Low confidence pixels are given a small weight while high confidence ones contribute largely in calculating the loss. This technique helps further reduce noise brought by inaccurate pseudo labels.

\begin{figure}[H]
\centering
\includegraphics[width=0.5\textwidth]{fig/confidence.pdf} 
\caption{Left figure: one RGB image; right figure: corresponding weight value $\omega$ of each pixel.} 
\label{fig:conf} 
\end{figure}

\subsection{Event Classification}
The AudioSet and VGGSound are both audio-visual datasets for event classification. We take a mini common set of them including 3710 data in AudioSet and 3748 data for training and 1937 data for testing in VGGSound with 46 event categories. VGGSound guarantees the audio-video correspondence as the sound source is visually evident within the video, while AudioSet does not. Therefore, we consider AudioSet as a unimodal dataset and VGG Sound as multimodal. Audios from AudioSet and audio-video pairs from VGGSound are taken as the labeled unimodal dataset $D_l$ and unlabeled multimodal data $D_u$ respectively. Similarly, a student network is given soft pseudo labels of the UM teacher for training.

==> supp2-exp.tex <==
\section{Experimental Results}
\subsection{Emotion Recognition}
One interesting finding is presented in Figure \ref{fig:emo}. We compare the confusion matrix that the UM teacher, NOISY student and our MM student generates on test data. Compared with NOISY student, the MM student contributes quite differently for 8 classes: it significantly improves the class ``surprised'' and slightly improves over the ``neutral'' class. We hypothesize that audios belonging to class ``surprised'' have more distinct features than ``neutral'', and a multi-modal student effectively utilizes this information.

\subsection{Semantic Segmentation}
Figure \ref{fig:seg} presents more segmentation results on NYU Depth V2 test data. We can see that the UM Teacher generates inconsistent and noisy predictions, for instance, they fail to identify sofas in the third, fourth and sixth example. NOISY Student improves a little over the teacher's prediction. However, its prediction is still messy. In contrast, MM student identifies the sofa as a whole and gives mostly correct predictions. Depth modality here enables knowledge expansion from the RGB teacher.

\subsection{Event Classification}
\begin{table}[h]\small
	%\renewcommand\tabcolsep{1pt}
	\centering
	\begin{tabular}{cccc}
		\toprule		
		& \multicolumn{3}{c}{Test mAP} \\
		&\makecell[c]{UM \\teacher}& \makecell[c]{NOISY \\student}&\makecell[c]{MM\\ student (ours)}\\
		\midrule
        % \rowcolor{mygray}
		basketball bounce&0.178& 0.263&0.542 \\
	    dog growling&0.069 & 0.096&0.516 \\
	   % \rowcolor{mygray}
	    people belly laughing& 0.334& 0.475 &0.800 \\
	    sliding door&0.104&0.163&0.388\\
	   % \rowcolor{mygray}
	    lawn mowing&0.318 &0.481 &0.541\\
		\bottomrule
	\end{tabular}
	\caption{Performance of top 5 event categories that MM student improves. Test mAP of the UM teacher and NOISY student are shown for comparison.}
	\label{tab:eventimprove}
\end{table}

\begin{figure*}[!htp]
\centering
\subfloat[RGB images]{
\begin{minipage}[b]{0.15\textwidth}
\centering
\includegraphics[scale=0.2]{./fig/seg/46/img.pdf} \\
\includegraphics[scale=0.2]{./fig/seg/280/img.pdf} \\
\includegraphics[scale=0.2]{./fig/seg/590/img.pdf} \\
\includegraphics[scale=0.2]{./fig/seg/618/img.pdf} \\
\includegraphics[scale=0.2]{./fig/seg/1108/img.pdf} \\
\includegraphics[scale=0.2]{./fig/seg/1313/img.pdf} \\
\end{minipage}
}\hspace{-1.5mm}
\subfloat[depth images]{
\begin{minipage}[b]{0.15\textwidth}
\centering
\includegraphics[scale=0.2]{./fig/seg/46/hha.pdf} \\
\includegraphics[scale=0.2]{./fig/seg/280/hha.pdf} \\
\includegraphics[scale=0.2]{./fig/seg/590/hha.pdf} \\
\includegraphics[scale=0.2]{./fig/seg/618/hha.pdf} \\
\includegraphics[scale=0.2]{./fig/seg/1108/hha.pdf} \\
\includegraphics[scale=0.2]{./fig/seg/1313/hha.pdf}
\end{minipage}
}\hspace{-1.5mm}
\subfloat[ground truth]{
\begin{minipage}[b]{0.15\textwidth}
\centering
\includegraphics[scale=0.2]{./fig/seg/46/gt.pdf} \\
\includegraphics[scale=0.2]{./fig/seg/280/gt.pdf} \\
\includegraphics[scale=0.2]{./fig/seg/590/gt.pdf} \\
\includegraphics[scale=0.2]{./fig/seg/618/gt.pdf} \\
\includegraphics[scale=0.2]{./fig/seg/1108/gt.pdf} \\
\includegraphics[scale=0.2]{./fig/seg/1313/gt.pdf} 
\end{minipage}
}\hspace{-1.5mm}
\subfloat[MM student (ours)]{
\begin{minipage}[b]{0.15\textwidth}
\centering
\includegraphics[scale=0.2]{./fig/seg/46/mmstudent.pdf} \\
\includegraphics[scale=0.2]{./fig/seg/280/mmstudent.pdf} \\
\includegraphics[scale=0.2]{./fig/seg/590/mmstudent.pdf} \\
\includegraphics[scale=0.2]{./fig/seg/618/mmstudent.pdf} \\
\includegraphics[scale=0.2]{./fig/seg/1108/mmstudent.pdf} \\
\includegraphics[scale=0.2]{./fig/seg/1313/mmstudent.pdf}
\end{minipage}
}\hspace{-1.5mm}
\subfloat[UM teacher]{
\begin{minipage}[b]{0.15\textwidth}
\centering
\includegraphics[scale=0.2]{./fig/seg/46/teacher.pdf} \\
\includegraphics[scale=0.2]{./fig/seg/280/teacher.pdf} \\
\includegraphics[scale=0.2]{./fig/seg/590/teacher.pdf} \\
\includegraphics[scale=0.2]{./fig/seg/618/teacher.pdf} \\
\includegraphics[scale=0.2]{./fig/seg/1108/teacher.pdf} \\
\includegraphics[scale=0.2]{./fig/seg/1313/teacher.pdf} 
\end{minipage}
}\hspace{-2mm}
\subfloat[NOISY student]{
\begin{minipage}[b]{0.15\textwidth}
\centering
\includegraphics[scale=0.2]{./fig/seg/46/noisystudent.pdf} \\
\includegraphics[scale=0.2]{./fig/seg/280/noisystudent.pdf} \\
\includegraphics[scale=0.2]{./fig/seg/590/noisystudent.pdf} \\
\includegraphics[scale=0.2]{./fig/seg/618/noisystudent.pdf} \\
\includegraphics[scale=0.2]{./fig/seg/1108/noisystudent.pdf} \\
\includegraphics[scale=0.2]{./fig/seg/1313/noisystudent.pdf} \\
\end{minipage}
}\hspace{-1.5mm}
\caption{Qualitative segmentation results on NYU Depth V2 test set.}
\label{fig:seg}
\end{figure*}

We list top 5 event categories that our MM student improves most in Table \ref{tab:eventimprove}. While NOISY student leads to similar performance gain for each event class, our MM student greatly improves over these classes with the assistance of video modality. For instance, the UM teacher performs poorly on the ``dog growling'' class with audio inputs only. NOISY student improves test mAP from 0.069 to 0.096 with the help of more data. In contrast, a MM student achieves an mAP of 0.542 and shows great improvement over the unimodal baselines. Video modality helps our MM student denoise these incorrect predictions given by the UM teacher.

==> supp3-ablation.tex <==
\section{Ablation Studies}
In this section, we provide a comprehensive study of various factors in \textit{MKE}. 
\subsection{Regularization}
The ablation study for regularization terms is provided in the main paper. We report performance of MM student (no reg), \ie, a MM student without regularization in all experiments. Results consistently show that a MM student yields better results than a MM student (no reg). We arrive at the conclusion that multimodality combined with regularization leads to best performance compared with all the baselines.

\subsection{Unlabeled Data Size}
We study the effect of unlabeled data size in this section. Specifically, for the task of semantic segmentation, we reduce unlabeled data size from 1488 RGB-D image pairs as reported in the main paper to 744 image pairs. Results are shown in Table \ref{tab:seg}. 

\renewcommand\arraystretch{1.0}
\begin{table}[H]
\centering
\begin{tabular}{ccccc}
\toprule
\multirow{2}*{Method} & \multicolumn{3}{c}{Train data} & \multirow{2}*{\makecell[c]{Test mIoU \\(\%)}} \\
~ & \textit{mod} & $D_l$ & $\tilde{D}_u$ &  ~ \\
\midrule
UM teacher & $rgb$ & $\checkmark$ & & 44.15  \\
UM student & $rgb$ &  &$\checkmark$  & 44.57  \\
NOISY student & $rgb$ & $\checkmark$ & $\checkmark$ & 46.85  \\
\makecell[c]{MM student (ours)}& $rgb, d$ & & $\checkmark$ & \textbf{47.44}  \\
\bottomrule
\end{tabular}
\caption{Results of semantic segmentation on NYU Depth V2. We set unlabeled data size smaller than labeled data size.}
\label{tab:seg}
\end{table}

UM student yields marginal improvement over UM teacher as it receives a small amount of unlabeled data and pseudo labels for training. On the contrary, provided with same data as the UM student, a MM student still achieves a mIoU gain of 3.29\%. Furthermore, although training data of NOISY student is twice greater than that of a MM student, half of which contain true labels, our MM student still achieves better results with respect to NOISY student. The great denoising capability of \textit{MKE} is thus shown.

\subsection{Teacher Model}
The UM teacher of previous experiments on NYU Depth V2 is implemented as DeepLab V3+. In this section, we experiment with the teacher model as RefineNet. We utilize same data as in Section 4.2, where $|D_l|=795$, $|D_u|=744$, and $|D_{test}|=654$. Table \ref{tab:ablation-teacher} reports performance when the UM teacher is RefineNet with ResNet-50 and ResNet-101 as backbone respectively. 

\renewcommand\arraystretch{1.0}
\begin{table}[H]
\centering
\begin{tabular}{cccc}
\toprule
\multirow{2}*{Method} & \multirow{2}*{\textit{mod}} & \multicolumn{2}{c}{Test mIoU(\%)} \\
~&~& \makecell[c]{RefineNet-\\Res50}& \makecell[c]{RefineNet-\\Res101}  \\
\midrule
UM teacher & $rgb$ & 42.41 & 44.18  \\
UM student & $rgb$ & 41.23 & 42.89  \\
NOISY student & $rgb$ & 43.21 & 45.69 \\
MM student & $rgb, d$ & \textbf{45.71} & \textbf{46.95}  \\
\bottomrule
\end{tabular}
\caption{Ablation study for UM teacher model architecture. MM student consistently denoises pseudo labels when teacher model varies.} 
\label{tab:ablation-teacher}
\end{table}

\renewcommand\arraystretch{1.0}
\begin{table}[!htbp]
\centering
\begin{tabular}{cccc}
\toprule
Method & \textit{mod} & \makecell[c]{Labels for \\distilling} & Test mIoU(\%) \\
\midrule
UM teacher & $rgb$ & $\star$ & 44.18  \\
UM student & $rgb$ & hard  & 42.53  \\
UM student & $rgb$ & soft & 42.89  \\
MM student & $rgb, d$ & hard & 46.64   \\
MM student & $rgb, d$ & soft & \textbf{46.95}  \\
\bottomrule
\end{tabular}
\caption{Ablation study for hard \textit{vs.} soft labels on semantic segmentation. $\star$ means that the UM teacher is trained on true labels. Other methods are trained on pseudo labels generated by the UM teacher.} 
\label{tab:ablation-labels}
\end{table}

Despite different model architectures of the UM teacher, the conclusion holds same: MM student significantly outperforms the UM teacher and UM student, achieving knowledge expansion. In addition, a stronger teacher (\ie, more reliable pseudo labels) will lead to a better student model in the case of both unimodality and multimodality. Another observation here is that UM student fails to surpass UM teacher due to limited size of $D_u$. On the contrary, given small amount of unlabeled data, our MM student effectively utilizes unlabeled multimodal data and outperforms NOISY student which has access to both labeled and unlabeled data.


\subsection{Pseudo Labels for Distilling}

We also investigate how soft and hard pseudo labels influence results and report results in Table \ref{tab:ablation-labels}. We follow same data and model settings in the previous section.

As shown in Table \ref{tab:ablation-labels}, soft labels yield slightly better results than hard labels. The MM student learning from soft labels of the UM teacher achieves highest test mIoU. 



==> supp4-proof.tex <==
\section{Proofs}
\subsection{Equivalence of Loss Terms}
We prove below that Equation (\ref{eq:eqv}) is equivalent to Equation (3) in the main paper.
\begin{equation}
    \theta_s^\star = \argmin_{\theta_s} \frac1 M \sum_{i=1}^M l_{cls}(\tilde{\mathbf{y}}_i, \mathcal{T}(\mathbf{f}_s(\mathbf{x}_i^\alpha, \mathbf{x}_i^\beta;\theta_s))
\label{eq:eqv}
\end{equation}

$l_{cls}$ refers to cross entropy loss for hard labels and KL divergence loss for soft labels. It takes the form of:
\begin{equation}
    \begin{aligned}
        l_{cls}(y, p) = - \sum_{k=1}^{K} y_k \log \frac{\exp{p_k}}{\sum_{j=1}^{K} \exp{p_j}} + \sum_{k=1}^{K} y_k \log {y_k}
    \end{aligned}
\end{equation}
where $y$ and $p$ are $K$-dimensional vectors. $K$ denotes the number of classes. For simplicity, let  $z$ denote the output of feeding $p$ into a softmax layer, \ie, $\forall k\in [K], z_k = \frac{\exp{p_k}}{\sum_{j=1}^{K} \exp{p_j}}$. 
\vspace{1mm}

The derivative of $l_{cls}(y, p)$ with respect to $p_j$ is:
\begin{equation}
\begin{aligned}
    \frac{\partial{l_{cls}(y, p)}} {\partial{p_j}} &= -\sum_{k=1}^{K} y_k \frac{\partial{\log{z_k}}} {\partial{p_j}} \\
    & = -\sum_{k=1}^{K} y_k (I_{kj} - z_j) = z_j - y_j
\end{aligned}
\end{equation}

Therefore, $\triangledown {l_{cls}} = [z_1-y_1, z_2-y_2, ..., z_k-y_k]$.
\begin{equation}
    ||\triangledown {l_{cls}}|| = \sqrt{\sum_{j=1}^K (y_j-z_j)^2} \leq \sqrt{K}
    \label{eq:lip}
\end{equation}

Equation (\ref{eq:lip}) states that $l_{cls}(y, p)$ is Lipschitz continuous in $p$ for fixed $y$ with respect to $||\cdot||$, where $\sqrt{K}$ is the Lipschitz constant. Therefore, $\exists -\sqrt{K} \leq \gamma \leq \sqrt{K}$, such that loss terms in Equation (\ref{eq:eqv}) equal to that of Equation (3) in the main paper.

\subsection{Lemma 1}
To start with, by definition of ($a, c$) expansion and $max(c_1,c_2)\leq\frac{1}{\bar{a}}$, we derive Equation (\ref{eq:ac1}) and (\ref{eq:ac2}) from Equation (10) and (11) in the main paper.
\begin{equation}
    \label{eq:ac1}
    \begin{aligned}
	P_i(N(V^{\alpha})) & \geq c_1 P_i(V^{\alpha}) \\
&\forall \ V^{\alpha} \subseteq \mathcal X^{\alpha} \ with \ P_i(V^{\alpha}) \leq \bar{a}
\end{aligned}
\end{equation}

\begin{equation}
    \label{eq:ac2}
    \begin{aligned}
P_i(N(V^{\beta})) & \geq c_2 P_i(V^{\beta}) \\
&\forall \ V^{\beta} \subseteq \mathcal X^{\beta} \ with \ P_i(V^{\beta}) \leq \bar{a}
\end{aligned}
\end{equation}

Multiplying both sides of Equation (\ref{eq:ac1}) and Equation (\ref{eq:ac2}), we have:
\begin{equation}
    \label{eq:acmid}
    \begin{aligned}
	P_i(N(V^{\alpha}))& P_i(N(V^{\beta})) \geq c_1 c_2 P_i(V^{\alpha})P_i(V^{\beta}) \\
&\forall \ V^{\alpha} \subseteq \mathcal X^{\alpha} \ with \ P_i(V^{\alpha}) \leq \bar{a} \\
&\forall \ V^{\beta} \subseteq \mathcal X^{\beta} \ with \ P_i(V^{\beta}) \leq \bar{a}
\end{aligned}
\end{equation}

Plugging in conditional independence (\ie, Equation (12) in the main paper) gives us:  
\begin{equation}
    \label{eq:acfinal}
    \begin{aligned}
         P_i(N(V)) & \geq c_1 c_2 P_i(V), \\
         & \forall \ V \subseteq \mathcal X \ with \ P_i(V) \leq \bar{a}
    \end{aligned}
\end{equation}

Thus, $P$ on $\mathcal X$ satisfies ($\bar{a}, c_1c_2$) expansion.
